Artist-Created Mesh Generation from Raw Observation

We present an end-to-end framework for generating artist-style meshes from noisy or incomplete point clouds, such as those captured by real-world sensors like LiDAR or mobile RGB-D cameras. Artist-created meshes are crucial for commercial graphics pipelines due to their compatibility with animation and texturing tools and their efficiency in rendering. However, existing approaches often assume clean, complete inputs or rely on complex multi-stage pipelines, limiting their applicability in real-world scenarios. To address this, we propose an end-to-end method that refines the input point cloud and directly produces high-quality, artist-style meshes. At the core of our approach is a novel reformulation of 3D point cloud refinement as a 2D inpainting task, enabling the use of powerful generative models. Preliminary results on the ShapeNet dataset demonstrate the promise of our framework in producing clean, complete meshes.

==> sec/04-datasets.tex <==
\section{Dataset}
\label{sec:dataset}


Our initial dataset for training and evaluation is constructed from ShapeNet for its high data quality within limited categories. We intend to use it as a clean starting point, then progressively fuse meshes from the other repositories. We follow \cite{chen2024meshanything} to filter out meshes with more than 800 faces and manually discarded low quality meshes by checking geometric integrity, annotation completeness, and category balance. This produces roughly 5k meshes. 
% We then reorder the mesh sequence following the convention adopted by \cite{hao2024meshtron}. This convention has three levels:
% \begin{enumerate}
%     \item \textit{Coordinate level}: Vertices are arranged in $yzx$ order, where $y$ represents the vertical axis.
%     \item \textit{Vertex level}: vertices within each face are sorted lexicographically, wht the lowest $yzx$-ordered vertex first.
%     \item \textit{Face level}: faces are sorted in ascending $yzx$-order based on the sorted values of their vertices.
% \end{enumerate}

The point clouds generated thus far are high-quality, free from corruption and noise. However, to simulate the challenges posed by real-world lidar data—namely, occlusion and measurement noise—we introduce a synthetic corruption procedure. Specifically, we randomly crop a portion of the point cloud to mimic occlusion and add Gaussian noise to the remaining points to simulate sensor inaccuracies. Our random cropping consists of two strategies: 1) randomly select $20\%$ to crop, and 2) crop $20\%$ of the points around a center region. While this procedure approximates real-world conditions, it may not fully capture the true distribution of lidar artifacts, suggesting a direction for future improvement, such as using a visibility mask to crop out points. After obtaining the point cloud, we extract its corresponding atlas, i.e., position map and normal map, for fine-tuning the Latent Diffusion.

Our dataset contains approximately 5.5k samples, split into $90\%$ for training and $10\%$ for testing, following the convention in \cite{meshanything}. Each sample consists of a clean point cloud, a synthetically corrupted counterpart, and their corresponding atlases. 
% Representative examples are shown in Fig. \ref{fig:dataset}.
\input{imgs/qualitative_result}
